The REBELS ALMA Survey: cosmic dust temperature evolution out to z $\sim$ 7

ALMA observations have revealed the presence of dust in the first generations of galaxies in the Universe. However, the dust temperature $T_d$ remains mostly unconstrained due to the few available FIR continuum data at redshift $z>5$. This introduces large uncertainties in several properties of high-$z$ galaxies, namely their dust masses, infrared luminosities, and obscured fraction of star formation. Using a new method based on simultaneous [CII] 158$\mu$m line and underlying dust continuum measurements, we derive $T_ d$ in the continuum and [CII] detected $z\approx 7$ galaxies in the ALMA Large Project REBELS sample. We find $39\ \mathrm{K} < T_d < 58\ \mathrm{K}$, and dust masses in the narrow range $M_d = (0.9-3.6)\times 10^7 M_{\odot}$. These results allow us to extend for the first time the reported $T_d(z)$ relation into the Epoch of Reionization. We produce a new physical model that explains the increasing $T_ d(z)$ trend with the decrease of gas depletion time, $t_{dep}=M_g/\mathrm{SFR}$, induced by the higher cosmological accretion rate at early times; this hypothesis yields $T_d \propto (1+z)^{0.4}$. The model also explains the observed $T_d$ scatter at a fixed redshift. We find that dust is warmer in obscured sources, as a larger obscuration results in more efficient dust heating. For UV-transparent (obscured) galaxies, $T_d$ only depends on the gas column density (metallicity), $T_d \propto N_H^{1/6}$ ($T_d \propto Z^{-1/6}$). REBELS galaxies are on average relatively transparent, with effective gas column densities around $N_H \simeq (0.03-1)\times 10^{21} \mathrm{cm}^{-2}$. We predict that other high-$z$ galaxies (e.g. MACS0416-Y1, A2744-YD4), with estimated $T_d \gg 60$ K, are significantly obscured, low-metallicity systems. In fact $T_d$ is higher in metal-poor systems due to their smaller dust content, which for fixed $L_{ IR}$ results in warmer temperatures.

==> additional_tex_files/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother

